The VoiceMOS Challenge 2022

We present the first edition of the VoiceMOS Challenge, a scientific event that aims to promote the study of automatic prediction of the mean opinion score (MOS) of synthetic speech. This challenge drew 22 participating teams from academia and industry who tried a variety of approaches to tackle the problem of predicting human ratings of synthesized speech. The listening test data for the main track of the challenge consisted of samples from 187 different text-to-speech and voice conversion systems spanning over a decade of research, and the out-of-domain track consisted of data from more recent systems rated in a separate listening test. Results of the challenge show the effectiveness of fine-tuning self-supervised speech models for the MOS prediction task, as well as the difficulty of predicting MOS ratings for unseen speakers and listeners, and for unseen systems in the out-of-domain setting.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> tables/metrics-correlations-all-tight.tex <==
\addtolength{\tabcolsep}{-3pt}
\begin{table}[h]
\centering
\caption{Linear correlation coefficients between different metrics, using the main track results.}
\label{tab:metrics-correlations-paper}

	\scriptsize


\hspace*{-30pt}

\begin{tabular}{ | c c | c c c c | c c c c | }
        \hline
         & & \multicolumn{4}{c|}{Utterance level} & \multicolumn{4}{c|}{System level} \\
         & & MSE & LCC & SRCC & KTAU & MSE & LCC & SRCC & KTAU \\
         \hline \hline
\multirow{4}{*}[0pt]{\makecell{Utt.\\level}} & MSE & 1.00 & -.955 & -.958 & -.955 & .906 & -.931 & -.932 & -.942 \\
& LCC & - & 1.00 & .999 & .997 & -.838 & .964 & .959 & .974 \\
& SRCC & - & - & 1.00 & .997 & -.835 & .962 & .959 & .974 \\
& KTAU & - & - & - & 1.00 & -.829 & .949 & .944 & .965\\
\hline
\multirow{4}{*}[0pt]{\makecell{Sys.\\level}} & MSE & - & - & - & - & 1.00 & -.875 & -.862 & -.870 \\
& LCC & - & - & - & - & - & 1.00 & .997 & .994\\
& SRCC & - & - & - & - & - & - & 1.00 & .994\\
& KTAU & - & - & - & - & - & - & - & 1.00\\


\hline
\end{tabular}
\end{table}
\addtolength{\tabcolsep}{3pt}

==> tables/raw-results.tex <==
% \begin{table}[t]
% 	\centering
% 	%\captionsetup{justification=centering}
% 	\caption{Main track evaluation results and the ranking of each team. Table order based on system level SRCC. For MSE, the smaller the better; for LCC, SRCC and KTAU, the larger the better. }
% 	\scriptsize
% % 	\footnotesize
%     % \tiny
	
% 	\centering
% % 	\hspace*{-0.3cm}
%     \hspace*{-10pt}
% 	\begin{tabular}{ | c | c c c c | c c c c | }
% % 		\toprule
%         \hline
% 		\multirow{2}{*}[0pt]{ID} & \multicolumn{4}{c|}{Utterance level} & \multicolumn{4}{c|}{System level} \\
% 		\cline{2-9}
% %		\cmidrule(lr){4-6} \cmidrule(lr){7-9}
% 		& MSE & LCC & SRCC & KTAU & MSE & LCC & SRCC & KTAU \\
% % 		\midrule
%         \hline
%         T11	& 0.179 & 0.895 & 0.894 & 0.725 & 0.101 & 0.941 & 0.939 & 0.797\\
%         T19 & 0.187 & 0.890 & 0.889 & 0.719 & 0.091 & 0.940 & 0.938 & 0.792 \\
% T17 & 0.165 & 0.900 & 0.897 & 0.730 & 0.090 & 0.939 & 0.936 & 0.794 \\
% T20 & 0.197 & 0.889 & 0.890 & 0.722 & 0.108 & 0.936 & 0.935 & 0.790\\
% T07 & 0.242 & 0.877 & 0.872 & 0.698 & 0.098 & 0.936 & 0.933 & 0.783\\
% T12 & 0.171 & 0.895 & 0.893 & 0.725 & 0.095 & 0.936 & 0.933 & 0.782\\
% T10 & 0.197 & 0.884 & 0.884 & 0.712 & 0.106 & 0.933 & 0.931 & 0.785\\
% T05 & 0.194 & 0.884 & 0.884 & 0.712 & 0.107 & 0.931 & 0.930 & 0.781\\
% T18 & 0.213 & 0.882 & 0.884 & 0.712 & 0.130 & 0.925 & 0.929 & 0.783\\
% T02 & 0.205 & 0.878 & 0.877 & 0.701 & 0.116 & 0.927 & 0.925 & 0.776\\
% T06 & 0.238 & 0.861 & 0.860 & 0.686 & 0.143 & 0.923 & 0.922 & 0.773\\
% B01 & 0.277 & 0.869 & 0.869 & 0.690 & 0.148 & 0.924 & 0.921 & 0.769\\
% T21 & 0.217 & 0.867 & 0.866 & 0.687 & 0.103 & 0.920 & 0.918 & 0.763\\
% T01 & 0.208 & 0.875 & 0.878 & 0.704 & 0.122 & 0.916 & 0.915 & 0.767\\
% T22 & 0.220 & 0.867 & 0.864 & 0.687 & 0.134 & 0.912 & 0.911 & 0.749\\
% T08 & 0.263 & 0.838 & 0.838 & 0.652 & 0.142 & 0.908 & 0.911 & 0.747\\
% T13 & 0.299 & 0.856 & 0.854 & 0.674 & 0.245 & 0.909 & 0.910 & 0.745\\
% T16 & 0.313 & 0.835 & 0.829 & 0.647 & 0.142 & 0.911 & 0.906 & 0.745\\
% T09 & 0.276 & 0.823 & 0.822 & 0.634 & 0.137 & 0.904 & 0.902 & 0.734\\
% B02 & 0.309 & 0.809 & 0.811 & 0.621 & 0.162 & 0.899 & 0.900 & 0.729\\
% T04 & 0.351 & 0.805 & 0.806 & 0.619 & 0.194 & 0.890 & 0.890 & 0.719\\
% B03 & 0.334 & 0.787 & 0.785 & 0.599 & 0.178 & 0.873 & 0.873 & 0.691\\
% T14 & 0.414 & 0.748 & 0.747 & 0.562 & 0.249 & 0.837 & 0.834 & 0.649\\
% T15 & 0.442 & 0.760 & 0.758 & 0.572 & 0.253 & 0.833 & 0.827 & 0.640\\

% % 		\bottomrule
%         \hline
% 	\end{tabular}
% 	\label{tab:main-track-results}
% 	\vspace*{-0.3cm}
% \end{table}

% \begin{table}[t]
% 	\centering
% 	%\captionsetup{justification=centering}
% 	\caption{OOD track evaluation results and the ranking of each team. Table order based on system level SRCC. For MSE, the smaller the better; for LCC, SRCC and KTAU, the larger the better. }
% 	\scriptsize
% % 	\footnotesize
%     % \tiny
	
% 	\centering
% % 	\hspace*{-0.3cm}
%     % \hspace*{-10pt}
% 	\begin{tabular}{ | c | c c c c | c c c c | }
% % 		\toprule
%         \hline
% 		\multirow{2}{*}[0pt]{ID} & \multicolumn{4}{c|}{Utterance level} & \multicolumn{4}{c|}{System level} \\
% 		\cline{2-9}
% %		\cmidrule(lr){4-6} \cmidrule(lr){7-9}
% 		& MSE & LCC & SRCC & KTAU & MSE & LCC & SRCC & KTAU \\
% % 		\midrule
%         \hline
%         T17 & 0.162 & 0.917 & 0.893 & 0.716 & 0.030 & 0.988 & 0.979 & 0.908\\
% T05 & 0.270 & 0.881 & 0.857 & 0.672 & 0.104 & 0.968 & 0.975 & 0.877\\
% B01 & 0.260 & 0.888 & 0.849 & 0.664 & 0.099 & 0.971 & 0.975 & 0.889\\
% T18 & 0.189 & 0.900 & 0.875 & 0.692 & 0.054 & 0.972 & 0.973 & 0.883\\
% T06 & 0.719 & 0.874 & 0.848 & 0.662 & 0.538 & 0.957 & 0.970 & 0.871\\
% T19 & 0.210 & 0.888 & 0.859 & 0.676 & 0.070 & 0.960 & 0.969 & 0.871\\
% T20 & 0.360 & 0.858 & 0.837 & 0.649 & 0.141 & 0.964 & 0.956 & 0.846\\
% T07 & 0.285 & 0.885 & 0.850 & 0.667 & 0.132 & 0.964 & 0.956 & 0.858\\
% B02 & 0.284 & 0.853 & 0.806 & 0.616 & 0.071 & 0.967 & 0.954 & 0.846\\
% T11 & 0.163 & 0.921 & 0.895 & 0.722 & 0.048 & 0.982 & 0.952 & 0.852\\
% T12 & 0.254 & 0.894 & 0.863 & 0.674 & 0.107 & 0.968 & 0.936 & 0.809\\
% B03 & 0.287 & 0.844 & 0.787 & 0.592 & 0.091 & 0.952 & 0.934 & 0.791\\
% T10 & 0.220 & 0.884 & 0.852 & 0.664 & 0.085 & 0.955 & 0.930 & 0.778\\
% T03 & 0.216 & 0.896 & 0.870 & 0.683 & 0.066 & 0.976 & 0.929 & 0.803\\
% T15 & 0.334 & 0.849 & 0.814 & 0.619 & 0.163 & 0.950 & 0.917 & 0.778\\
% T22 & 0.261 & 0.885 & 0.834 & 0.646 & 0.107 & 0.957 & 0.904 & 0.785\\
% T02 & 3.619 & 0.415 & 0.460 & 0.336 & 3.393 & 0.469 & 0.527 & 0.446\\
% T21 & 2.516 & 0.440 & 0.429 & 0.305 & 2.261 & 0.491 & 0.516 & 0.385\\


% % 		\bottomrule
%         \hline
% 	\end{tabular}
% 	\label{tab:ood-track-results}
% 	\vspace*{-0.3cm}
% \end{table}

\begin{table*}[h!]
	\centering
	%\captionsetup{justification=centering}
	\caption{Evaluation results. Numbers in parenthesis are the rankings. For MSE, the smaller the better; for LCC, SRCC and KTAU, the larger the better. }
% 	\scriptsize
% 	\footnotesize
    \tiny
	
	\centering
% 	\hspace*{-0.3cm}
    \hspace*{-30pt}
	\begin{tabular}{ | c | c c c c | c c c c | c c c c | c c c c | }
% 		\toprule
        \hline
		\multirow{3}{*}[0pt]{ID} & \multicolumn{8}{c|}{Main track} & \multicolumn{8}{c|}{OOD track} \\
		\cline{2-17}
		& \multicolumn{4}{c|}{Utterance level} & \multicolumn{4}{c|}{System level} & \multicolumn{4}{c|}{Utterance level} & \multicolumn{4}{c|}{System level} \\
		\cline{2-17}
%		\cmidrule(lr){4-6} \cmidrule(lr){7-9}
		& MSE & LCC & SRCC & KTAU & MSE & LCC & SRCC & KTAU & MSE & LCC & SRCC & KTAU & MSE & LCC & SRCC & KTAU \\
% 		\midrule
        \hline
        B01 & 0.277 (17) & 0.869 (12) & 0.869 (12) & 0.690 (12) & 0.148 (18) & 0.924 (11) & 0.921 (12) & 0.769 (12) & 0.260 (8) & 0.888 (6) & 0.849 (10) & 0.664 (10) & 0.099 (9) & 0.971 (5) & 0.975 (2) & 0.889 (2) \\
B02 & 0.309 (19) & 0.809 (20) & 0.811 (20) & 0.621 (20) & 0.162 (19) & 0.899 (20) & 0.900 (20) & 0.729 (20) & 0.284 (11) & 0.853 (14) & 0.806 (15) & 0.616 (15) & 0.071 (6) & 0.967 (8) & 0.954 (9) & 0.846 (9) \\
B03 & 0.334 (21) & 0.787 (22) & 0.785 (22) & 0.599 (22) & 0.178 (20) & 0.873 (22) & 0.873 (22) & 0.691 (22) & 0.287 (13) & 0.844 (16) & 0.787 (16) & 0.592 (16) & 0.091 (8) & 0.952 (15) & 0.934 (12) & 0.791 (13) \\
\hline
T01 & 0.208 (9) & 0.875 (11) & 0.878 (9) & 0.704 (9) & 0.122 (11) & 0.916 (14) & 0.915 (14) & 0.767 (13) & - & - & - & - & - & - & - & \\
T02 & 0.205 (8) & 0.878 (9) & 0.877 (10) & 0.701 (10) & 0.116 (10) & 0.927 (9) & 0.925 (10) & 0.776 (10) & 3.619 (18) & 0.415 (18) & 0.460 (17) & 0.336 (17) & 3.393 (18) & 0.469 (18) & 0.527 (17) & 0.446 (17) \\
T03 & - & - & - & - & - & - & - & - & 0.216 (5) & 0.896 (4) & 0.870 (4) & 0.683 (4) & 0.066 (4) & 0.976 (3) & 0.929 (14) & 0.803 (12) \\
T04 & 0.351 (22) & 0.805 (21) & 0.806 (21) & 0.619 (21) & 0.194 (21) & 0.890 (21) & 0.890 (21) & 0.719 (21) & - & - & - & - & - & - & - & \\
T05 & 0.194 (5) & 0.884 (6) & 0.884 (7) & 0.712 (7) & 0.107 (8) & 0.931 (8) & 0.930 (8) & 0.781 (9) & 0.270 (10) & 0.881 (11) & 0.857 (7) & 0.672 (7) & 0.104 (10) & 0.968 (6) & 0.975 (2) & 0.877 (4) \\
T06 & 0.238 (13) & 0.861 (15) & 0.860 (15) & 0.686 (15) & 0.143 (17) & 0.923 (12) & 0.922 (11) & 0.773 (11) & 0.719 (16) & 0.874 (12) & 0.848 (11) & 0.662 (11) & 0.538 (16) & 0.957 (12) & 0.970 (5) & 0.871 (5) \\
T07 & 0.242 (14) & 0.877 (10) & 0.872 (11) & 0.698 (11) & 0.098 (4) & 0.936 (4) & 0.933 (5) & 0.783 (6) & 0.285 (12) & 0.885 (9) & 0.850 (9) & 0.667 (8) & 0.132 (13) & 0.964 (9) & 0.956 (7) & 0.858 (7) \\
T08 & 0.263 (15) & 0.838 (17) & 0.838 (17) & 0.652 (17) & 0.142 (15) & 0.908 (18) & 0.911 (16) & 0.747 (16) & - & - & - & - & - & - & - & \\
T09 & 0.276 (16) & 0.823 (19) & 0.822 (19) & 0.634 (19) & 0.137 (14) & 0.904 (19) & 0.902 (19) & 0.734 (19) & - & - & - & - & - & - & - & \\
T10 & 0.197 (7) & 0.884 (7) & 0.884 (6) & 0.712 (8) & 0.106 (7) & 0.933 (7) & 0.931 (7) & 0.785 (5) & 0.220 (6) & 0.884 (10) & 0.852 (8) & 0.664 (9) & 0.085 (7) & 0.955 (14) & 0.930 (13) & 0.778 (15) \\
T11 & 0.179 (3) & 0.895 (2) & 0.894 (2) & 0.725 (3) & 0.101 (5) & 0.941 (1) & 0.939 (1) & 0.797 (1) & 0.163 (2) & 0.921 (1) & 0.895 (1) & 0.722 (1) & 0.048 (2) & 0.982 (2) & 0.952 (10) & 0.852 (8) \\
T12 & 0.171 (2) & 0.895 (3) & 0.893 (3) & 0.725 (2) & 0.095 (3) & 0.936 (6) & 0.933 (6) & 0.782 (8) & 0.254 (7) & 0.894 (5) & 0.863 (5) & 0.674 (6) & 0.107 (12) & 0.968 (7) & 0.936 (11) & 0.809 (11) \\
T13 & 0.299 (18) & 0.856 (16) & 0.854 (16) & 0.674 (16) & 0.245 (22) & 0.909 (17) & 0.910 (17) & 0.745 (18) & - & - & - & - & - & - & - & \\
T14 & 0.414 (23) & 0.748 (24) & 0.747 (24) & 0.562 (24) & 0.249 (23) & 0.837 (23) & 0.834 (23) & 0.649 (23) & - & - & - & - & - & - & - & \\
T15 & 0.442 (24) & 0.760 (23) & 0.758 (23) & 0.572 (23) & 0.253 (24) & 0.833 (24) & 0.827 (24) & 0.640 (24) & 0.334 (14) & 0.849 (15) & 0.814 (14) & 0.619 (14) & 0.163 (15) & 0.950 (16) & 0.917 (15) & 0.778 (15) \\
T16 & 0.313 (20) & 0.835 (18) & 0.829 (18) & 0.647 (18) & 0.142 (16) & 0.911 (16) & 0.906 (18) & 0.745 (17) & - & - & - & - & - & - & - & \\
T17 & 0.165 (1) & 0.900 (1) & 0.897 (1) & 0.730 (1) & 0.090 (1) & 0.939 (3) & 0.936 (3) & 0.794 (2) & 0.162 (1) & 0.917 (2) & 0.893 (2) & 0.716 (2) & 0.030 (1) & 0.988 (1) & 0.979 (1) & 0.908 (1) \\
T18 & 0.213 (10) & 0.882 (8) & 0.884 (8) & 0.712 (6) & 0.130 (12) & 0.925 (10) & 0.929 (9) & 0.783 (6) & 0.189 (3) & 0.900 (3) & 0.875 (3) & 0.692 (3) & 0.054 (3) & 0.972 (4) & 0.973 (4) & 0.883 (3) \\
T19 & 0.187 (4) & 0.890 (4) & 0.889 (5) & 0.719 (5) & 0.091 (2) & 0.940 (2) & 0.938 (2) & 0.792 (3) & 0.210 (4) & 0.888 (7) & 0.859 (6) & 0.676 (5) & 0.070 (5) & 0.960 (11) & 0.969 (6) & 0.871 (5) \\
T20 & 0.197 (6) & 0.889 (5) & 0.890 (4) & 0.722 (4) & 0.108 (9) & 0.936 (5) & 0.935 (4) & 0.790 (4) & 0.360 (15) & 0.858 (13) & 0.837 (12) & 0.649 (12) & 0.141 (14) & 0.964 (10) & 0.956 (7) & 0.846 (9) \\
T21 & 0.217 (11) & 0.867 (14) & 0.866 (13) & 0.687 (14) & 0.103 (6) & 0.920 (13) & 0.918 (13) & 0.763 (14) & 2.516 (17) & 0.440 (17) & 0.429 (18) & 0.305 (18) & 2.261 (17) & 0.491 (17) & 0.516 (18) & 0.385 (18) \\
T22 & 0.220 (12) & 0.867 (13) & 0.864 (14) & 0.687 (13) & 0.134 (13) & 0.912 (15) & 0.911 (15) & 0.749 (15) & 0.261 (9) & 0.885 (8) & 0.834 (13) & 0.646 (13) & 0.107 (11) & 0.957 (13) & 0.904 (16) & 0.785 (14) \\







        \hline
	\end{tabular}
	\label{tab:results}

\end{table*}
